Recurrent Additive Networks

We introduce recurrent additive networks (RANs), a new gated RNN which is distinguished by the use of purely additive latent state updates. At every time step, the new state is computed as a gated component-wise sum of the input and the previous state, without any of the non-linearities commonly used in RNN transition dynamics. We formally show that RAN states are weighted sums of the input vectors, and that the gates only contribute to computing the weights of these sums. Despite this relatively simple functional form, experiments demonstrate that RANs perform on par with LSTMs on benchmark language modeling problems. This result shows that many of the non-linear computations in LSTMs and related networks are not essential, at least for the problems we consider, and suggests that the gates are doing more of the computational work than previously understood.

==> architecture.tex <==

\section{Architecture}

Present our new architecture(s)

\begin{equation}
    r_t = \sigma (W_x x_t + W_h h_{t-1})
\end{equation}
\begin{equation}
    h_t = r_t \odot W_x x_t + (1 - r_t) \odot h_{t-1}
\end{equation}


Explain how they relate to previous ones

Present \& derive mathematical properties. Specifically:
\begin{equation}
    h_t = \sum^t_{i=1} v_i \odot x_i
\end{equation}
(Relate this property to attention.)

Present the unordered version based on the equation, and explain its difference.
\begin{equation}
    v_i = softmax(W_x x_t \odot W_h W_x x_i)
\end{equation}

Mention that it's expressive, for example, it can XOR.

==> background.tex <==

\section{Background: Recurrent Neural Networks}

Formally, an RNN encodes an arbitrary-length sequence of $d_x$-dimensional vectors $x_1, ..., x_n$ as a single $d_y$-dimensional vector $y_n$. It solves the problem of handling arbitrary-length sequences by recurrently reading a new input $x_t$ at each time step $t$, combining it with the network's previous state $h_{t-1}$ to produce a new state $h_t$, and emitting an output $y_t$. In most cases, $y_t = h_t$; hence, the sequence's encoding is typically the network's state when reading the last input ($h_n$).

The most basic RNN, which we refer to as \emph{SimpleRNN} \cite{RNN}, can be described by the following equation:
\begin{equation}
h_t = f(W_x x_t + W_h h_{t-1})
\end{equation}
where $f$ is some non-linearity (typically $tanh$). $W_x$ is a $d_{x} \times d_{h}$ matrix that projects the inputs into the hidden space, while $W_h$ is a $d_{h} \times d_{h}$ transition matrix. Together, they constitute the SimpleRNN's parameters. While relatively straightforward, this model was found to be quite difficult to train in practice, due to the problem of vanishing gradients \citet{vanishing}. \omer{We should explain in half a sentence what vangrad means.} \omer{Also, maybe change the notation of $W_x x_t$ to $e_t$?}

To address this issue, \citep{lstm} introduced a new type of RNN: \emph{long short-term memory} (LSTM). LSTMs contain various gating mechanisms that prevent some of the gradients from decaying too quickly. Specifically, ... \omer{add LSTM equations}
\begin{equation}
...
\end{equation}
While LSTMs have been successfully applied to virtually every NLP task \cite{} \omer{drop 2-3 pioneering applications, such as sutskever's translation}, their architecture is considerably more convoluted than SimpleRNNs', requiring 4 times as many parameters \omer{and NNN times more operations... think about some theoretical way to express the complexity/computation time}.

To simplify LSTMs, \cite{cho-gru} introduced \emph{gated recurrent units} (GRUs). \omer{dive into the exact details - which gates/actions were removed, referring to LSTM equations}. \omer{Present GRU equations}.
\begin{equation}
...
\end{equation}
Although GRUs are arguably simpler than LSTMs, they still require 3 times as many parameters \omer{and NNN times more operations} as SimpleRNNs.
\omer{One thing we *shouldn't* do: take a stand on the GRU vs LSTM performance debate. This is a minefield. We should stick to consensus facts such as simplicity, number of parameters, etc.}

In this work, we take the simplification process one step further, and present a new RNN that contains exactly the same number of parameters as a SimpleRNN, yet is able to match GRUs and LSTMs in performance on various NLP tasks.


==> cells.tex <==
\definecolor{g-red}{HTML}{DB4437}
\definecolor{g-blue}{HTML}{4285F4}
\definecolor{g-green}{HTML}{0F9D58}
\definecolor{g-yellow}{HTML}{F4B400}
\definecolor{g-orange}{HTML}{FF9800}
\definecolor{g-grey}{HTML}{9E9E9E}

\newcommand\unit[1] {
\draw[rounded corners, fill=g-green!30] (#1, 0) rectangle (#1 + 3, 3);
\draw[fill=g-orange!30] (#1 + 2.5,4) circle (0.3) node {$h_t$};
\draw[fill=g-blue!30] (#1 + 0.5,-1) circle (0.3) node {$x_t$};
}
\newcommand\lstm[1] {
\unit{#1}
\draw[rounded corners, fill=g-yellow] (#1 + 1, 1.5) rectangle (#1 + 1.5 + 0.5, 1.5 + 0.5) node at (#1 + 1, 1.5) {$\tanh$};
}

\begin{figure}
\centering

\begin{tikzpicture}
\lstm{0}
\end{tikzpicture}
\end{figure}
